Optimal Sample Selection Through Uncertainty Estimation and Its Application in Deep Learning

Modern deep learning heavily relies on large labeled datasets, which often comse with high costs in terms of both manual labeling and computational resources. To mitigate these challenges, researchers have explored the use of informative subset selection techniques, including coreset selection and active learning. Specifically, coreset selection involves sampling data with both input ($\bx$) and output ($\by$), active learning focuses solely on the input data ($\bx$). In this study, we present a theoretically optimal solution for addressing both coreset selection and active learning within the context of linear softmax regression. Our proposed method, COPS (unCertainty based OPtimal Sub-sampling), is designed to minimize the expected loss of a model trained on subsampled data. Unlike existing approaches that rely on explicit calculations of the inverse covariance matrix, which are not easily applicable to deep learning scenarios, COPS leverages the model's logits to estimate the sampling ratio. This sampling ratio is closely associated with model uncertainty and can be effectively applied to deep learning tasks. Furthermore, we address the challenge of model sensitivity to misspecification by incorporating a down-weighting approach for low-density samples, drawing inspiration from previous works. To assess the effectiveness of our proposed method, we conducted extensive empirical experiments using deep neural networks on benchmark datasets. The results consistently showcase the superior performance of COPS compared to baseline methods, reaffirming its efficacy.

==> materials.tex <==
\section{Old Lemmas}
\begin{lemma}
\begin{align*}
    \cL(\bar \beta) - \cL(\beta^*) = \bbE_{(\bmx, y) \sim \cD} \left[ w(\beta^*; \bmx)(\bmx^\top (\beta^* - \bar \beta))^2 + o(\bmx^\top(\beta^* - \bar \beta)) \right]
\end{align*} 
\end{lemma}
\begin{lemma}
\label{lamma:un_bias}
\begin{align*}
    \bbE_{\bar \cS | \cS}[(\bmx^\top(\hat \beta_\MLE - \bar \beta))] = 0
\end{align*}
\end{lemma}
\begin{proof}
\begin{align*}
    \bbE_{\bar \cS | \cS, \pi}[(\bmx^\top(\hat \beta_\MLE - \bar \beta))] = \bmx^\top ( \hat \beta_\MLE - \bbE_{ \bar \cS | \cS, \pi}[\bar \beta]) = 0
\end{align*}
\end{proof}
\begin{lemma}
    \begin{align*}
    \argmin_{\pi} \bbE_{\bar \cS|\cS, \pi}\left[\cL(\bar \beta; \cD) - \cL(\beta^*; \cD) \right] = \argmin_{\pi} \bbE_{\bar \cS|\cS, \pi}\left[ \bbE_{(\bmx, y) \sim \cD} \left[ w(\beta^*; \bmx)(\bmx^\top (\beta_\MLE - \bar \beta))^2 \right] \right]
    \end{align*}
\end{lemma}

\begin{proof}
    \begin{align*}
        & \argmin_{\pi} \bbE_{\bar \cS|\cS, \pi}\left[\bbE_{(\bmx, y) \sim \cD} \left[ w(\beta^*; \bmx)(\bmx^\top (\beta^* - \bar \beta))^2 \right]\right] \\
        = & \argmin_{\pi} \bbE_{\bar \cS|\cS, \pi}\left[\bbE_{(\bmx, y) \sim \cD} \left[ w(\beta^*; \bmx)(\bmx^\top (\beta^* - \hat \beta_\MLE +  \hat \beta_\MLE - \bar \beta))^2 \right]\right] \\
        = & \argmin_{\pi} \bbE_{\bar \cS|\cS, \pi}\left[\bbE_{(\bmx, y) \sim \cD} \left[ w(\beta^*; \bmx)\left((\bmx^\top (\beta^* - \hat \beta_\MLE))^2  + (\bmx^\top (\beta^* - \hat \beta_\MLE))(\bmx^\top(\hat \beta_\MLE - \bar \beta)) +  (\bmx^\top(\hat \beta_\MLE - \bar \beta))^2 \right) \right]\right].
    \end{align*}
We have 
\begin{align*}
    & \bbE_{\bar \cS | \cS, \pi} \left[ \bbE_{(\bmx, y) \sim \cD} \left[w(\beta^*; \bmx) (\bmx^\top (\beta^* - \hat \beta_\MLE))(\bmx^\top(\hat \beta_\MLE - \bar \beta))\right] \right] \\
    = & \bbE_{(\bmx, y) \sim \cD} \left[w(\beta^*; \bmx) (\bmx^\top (\beta^* - \hat \beta_\MLE))\bbE_{\bar \cS | \cS, \pi}[(\bmx^\top(\hat \beta_\MLE - \bar \beta))]\right] = 0.
\end{align*}
The last equation is due to Lemma \ref{lamma:un_bias}. We finish the proof by noting that $\hat \beta_\MLE$ does not depend on $\bar \cS$.  
\end{proof}
\begin{lemma}
[Theorem 2 of \cite{wang2018optimal}]
\label{lemma:beta_closeness}
If assumptions \ref{ass:ass1}-\ref{ass:ass3} hold, then as $n \xrightarrow[]{} \infty$ and $r \xrightarrow[]{} \infty$, conditional on $\cS$ in probability, 
\begin{align*}
    \bV^{-1/2}(\bar \beta - \hat \beta_\MLE) \xrightarrow[]{d} \cN(0, \bI),
\end{align*}
where $\xrightarrow[]{d}$ denotes convergence in distribution, and 
$$\bV = \bM_X^{-1}(\hat\beta_\MLE; \cS) \bV_c \bM_X^{-1}(\hat\beta_\MLE; \cS)$$ 
 $$
 \bV_c = \frac{1}{rn^2} \sum_{(\bmx, y) \in \cS} \frac{(y - p(\hat \beta_\MLE; \bmx))^2\bmx \bmx^\top}{\pi(\bmx)}
 $$     
\end{lemma}

\begin{thm}[Main theorem]
    \begin{align*}
        \bbE_{\bar \cS|\cS, \pi}\left[ \bbE_{(\bmx, y) \sim \cD} \left[ w(\beta^*; \bmx)(\bmx^\top (\hat \beta_\MLE - \bar \beta))^2 \right] \right] = \frac{1}{rn^2} \sum_{(\bmx, y) \in \cS} \frac{(y - p(\hat \beta_\MLE; \bmx))^2\|\bmx\|^2_{\bM_X(\hat\beta_\MLE; \cS)^{-1}}}{\pi(\bmx)} + o(1/n)
    \end{align*} 
 \end{thm}
 \begin{proof}
     \begin{align*}
         & \bbE_{\bar \cS|\cS, \pi}\left[ \bbE_{(\bmx, y) \sim \cD} \left[ w(\beta^*; \bmx)(\bmx^\top (\hat \beta_\MLE - \bar \beta))^2 \right] \right] \\
         = & \bbE_{(\bmx, y) \sim \cD} \left[ w(\beta^*; \bmx)\bmx^\top \bbE_{\bar \cS|\cS, \pi}[(\hat \beta_\MLE - \bar \beta) (\hat \beta_\MLE - \bar \beta)^\top] \bmx \right] \\
         = & \text{Trace}\left( \bbE_{(\bmx, y) \sim \cD} \left[ w(\beta^*; \bmx)\bmx\bmx^\top \right]\bbE_{\bar \cS|\cS, \pi}\left[(\hat \beta_\MLE - \bar \beta) (\hat \beta_\MLE - \bar \beta)^\top\right]\right)\\
         = & \text{Trace}\left( \bM_X(\beta^*; \cD)\bM_X^{-1}(\hat\beta_\MLE; \cS) \frac{1}{rn^2} \sum_{(\bmx, y) \in \cS} \frac{(y - p(\hat \beta_\MLE; \bmx))^2\bmx \bmx^\top}{\pi(\bmx)} \bM_X^{-1}(\hat\beta_\MLE; \cS)\right) \\
         = & \frac{1}{rn^2} \sum_{(\bmx, y) \in \cS} \frac{(y - p(\hat \beta_\MLE; \bmx))^2\bmx^\top \bM_X^{-1}(\hat\beta_\MLE; \cS) \bmx}{\pi(\bmx)} + o(1/n).
     \end{align*}
 \end{proof}
\begin{thm}[Main Coreset Sampling]
\begin{align*}
    \pi(\bmx) = \frac{|y - p(\hat \beta_\MLE; \bmx)|\|\bmx\|_{\bM_X(\hat\beta_\MLE; \cS)^{-1}}}{\sum_{(\bmx', y) \in \cS} |y - p(\hat \beta_\MLE; \bmx')|\|\bmx'\|_{\bM_X(\hat\beta_\MLE; \cS)^{-1}} }
\end{align*}
\end{thm}
\begin{proof}
\begin{align*}
    & \frac{1}{rn^2} \sum_{(\bmx, y) \in \cS} \frac{(y - p(\hat \beta_\MLE; \bmx))^2\|\bmx\|^2_{\bM_X(\hat\beta_\MLE; \cS)^{-1}}}{\pi(\bmx)} \\
    = & \frac{1}{rn^2} \sum_{(\bmx, y) \in \cS} \pi(\bmx) \sum_{(\bmx, y) \in \cS} \frac{(y - p(\hat \beta_\MLE; \bmx))^2\|\bmx\|^2_{\bM_X(\hat\beta_\MLE; \cS)^{-1}}}{\pi(\bmx)} \\
    \geq & \frac{1}{rn^2} \sum_{(\bmx, y) \in \cS} |y - p(\hat \beta_\MLE; \bmx)|\|\bmx\|_{\bM_X(\hat\beta_\MLE; \cS)^{-1}}
\end{align*}
The first equality is due to $\sum_{(\bmx, y) \in \cS} \pi(\bmx) = 1$. The last inequality is due to Cauchy-Schwarz inequality and the equliaty holds on when $\pi(\bmx) \propto |y - p(\hat \beta_\MLE; \bmx)|\|\bmx\|_{\bM_X(\hat\beta_\MLE; \cS)^{-1}}$. 
\end{proof}

\begin{thm}[Main theorem without $Y$]
    \begin{align*}
        & \bbE_{\bar \cS|\cS_X, \pi}\left[ \bbE_{(\bmx, y) \sim \cD} \left[ w(\beta^*; \bmx)(\bmx^\top (\hat \beta_\MLE - \bar \beta))^2 \right] \right] \\
        = & \frac{1}{rn^2} \sum_{(\bmx, y) \in \cS} \frac{\left(p(\beta^*; \bmx) - 2 p(\beta^*; \bmx) p(\hat \beta_\MLE; \bmx) + p(\hat \beta_\MLE; \bmx)^2\right)\|\bmx\|^2_{\bM_X(\hat\beta_\MLE; \cS)^{-1}}}{\pi(\bmx)} + o(1/n)
    \end{align*} 
Omitting the higher order term, the optimal sampling is as follows:
\begin{align*}
    \pi(\bmx) = \frac{\left(p(\beta^*; \bmx) - 2 p(\beta^*; \bmx) p(\hat \beta_\MLE; \bmx) + p(\hat \beta_\MLE; \bmx)^2\right)\|\bmx\|^2_{\bM_X(\hat\beta_\MLE; \cS)^{-1}}}{\sum_{(\bmx', y') \in \cS}\left(p(\beta^*; \bmx') - 2 p(\beta^*; \bmx') p(\hat \beta_\MLE; \bmx') + p(\hat \beta_\MLE; \bmx)^2\right)\|\bmx'\|^2_{\bM_X(\hat\beta_\MLE; \cS)^{-1}}}
\end{align*}
 \end{thm}
 \begin{proof}
 \begin{align*}
& \bbE_{\bar \cS|\cS_X, \pi}\left[ \bbE_{(\bmx, y) \sim \cD} \left[ w(\beta^*; \bmx)(\bmx^\top (\hat \beta_\MLE - \bar \beta))^2 \right] \right] \\
= & \bbE_{\cS_Y|\cS_X, \pi}\left[\bbE_{\bar \cS|\cS_X, \cS_Y, \pi}\left[ \bbE_{(\bmx, y) \sim \cD} \left[ w(\beta^*; \bmx)(\bmx^\top (\hat \beta_\MLE - \bar \beta))^2 \right] \right]\right] \\
= & \bbE_{\bar \cS|\cS_X, \cS_Y, \pi}\left[\frac{1}{rn^2} \sum_{(\bmx, y) \in \cS} \frac{(y - p(\hat \beta_\MLE; \bmx))^2\|\bmx\|^2_{\bM_X(\hat\beta_\MLE; \cS)^{-1}}}{\pi(\bmx)} + o(1/n)\right] \\
= & \frac{1}{rn^2} \sum_{(\bmx, y) \in \cS} \frac{\bbE_{y|\bmx}[(y - p(\hat \beta_\MLE; \bmx))^2]\|\bmx\|^2_{\bM_X(\hat\beta_\MLE; \cS)^{-1}}}{\pi(\bmx)} + o(1/n)
 \end{align*}
By noting that $\bbE_{y|\bmx} [y] = p(\beta^*; \bmx)$ and $\bbE_{y|\bmx} [y^2] = p(\beta^*; \bmx)$, we have  
\begin{align*}
    \bbE_{y|\bmx}[(y - p(\hat \beta_\MLE; \bmx))^2] = p(\beta^*; \bmx) - 2 p(\beta^*; \bmx) p(\hat \beta_\MLE; \bmx) + p(\hat \beta_\MLE; \bmx)^2.
\end{align*}
We finish the proof after plugin the result.
% \frac{1}{rn^2} \sum_{(\bmx, y) \in \cS} \frac{(y - p(\hat \beta_\MLE; \bmx))^2\|\bmx\|^2_{\bM_X(\hat\beta_\MLE; \cS)^{-1}}}{\pi(\bmx)} + o(1/n)    
 \end{proof}


\begin{thm}[Uncertainty Estimation]
\label{thm:uncertainty_estimation_app}
When $M,n \xrightarrow[]{} \infty$, we have $$n\mbox{Std}(\bmx)^2 \rightarrow \bmx^\top \bM_X^{-1}(\hbeta_{\MLE}; \cS) \bmx,$$
in probability.
\end{thm}

\begin{proof}
First of all, We write $\std^2$ as
\begin{align}\label{eq:std_decompose}
    \std^2 &= \frac{1}{M-1}\sum_{m=1}^M \Big(\bmx^\top\hbeta_m - \frac{1}{M}\sum_{j=1}^M\bmx^\top\hbeta_j \Big)^2\notag\\
    &= \frac{1}{M-1}\sum_{m=1}^M \Big(\bmx^\top(\hbeta_m - \beta^*) - \frac{1}{M}\sum_{j=1}^M\bmx^\top(\hbeta_j - \beta^*) \Big)^2\notag\\
    &= \frac{1}{M-1}\sum_{m=1}^M \Big( \bmx^\top(\hbeta_m - \beta^*) \Big)^2 - \frac{1}{M(M-1)} \Big( \sum_{m=1}^M\bmx^\top(\hbeta_j - \beta^*) \Big)^2\notag\\
    &= \underbrace{\frac{1}{M-1}\sum_{m=1}^M \Big( \bmx^\top(\hbeta_m - \beta^*) \Big)^2}_{Q_1} - \underbrace{\frac{M}{M-1}\big(\bmx^\top(\bar \beta - \beta^*)\big)^2}_{Q_2},
\end{align}
where we define the mean variable $\bar\beta=M^{-1}\sum_{m=1}^M\hbeta_m$. 

Then, we derive the convergence of the terms $Q_1$ and $Q_2$ in \eqref{eq:std_decompose} separately. For the term $Q_1$, since $(\bmx^\top(\hbeta_1 - \beta^*))^2,\ldots,(\bmx^\top(\hbeta_M - \beta^*))^2$ are i.i.d variables with a finite mean $\bbE[(\bmx^\top(\hbeta_1 - \beta^*))^2]$, we invoke the weak law of large numbers to get
\begin{align}\label{eq:std_Q1}
Q_1= \frac{M}{M-1}\cdot\frac{1}{M}\sum_{m=1}^M \Big( \bmx^\top(\hbeta_m - \beta^*) \Big)^2 \rightarrow \frac{M}{M-1} \bbE\big[(\bmx^\top(\hbeta_1 - \beta^*))^2\big],
\end{align}
in probability. Moreover, we know from \cite{ly2017tutorial} that as $n\rightarrow\infty$,
\begin{equation}\label{eq:normality}
\sqrt{n}\bmx^\top(\hbeta_m - \beta^*) \rightarrow N\big(0, \bmx^\top\bM_{X}^{-1}(\beta^*, \cD)\bmx\big)
\end{equation}
in distribution, which implies that
\begin{align*}
\sqrt{n}(\hat \beta_m- \beta^*) \rightarrow N(0, \bM_{X}^{-1}(\beta^*, \cD))
\end{align*}
in distribution.
Additionally, we find that for each $m\in[M]$, the $(\bmx^\top(\hbeta_1 - \beta^*))^2$ is upper bounded with a high probability due to $\|\hbeta_1-\beta^*\|_2=O_P(n^{-1/2})$. Then, we can invoke Theorem 25.12 in \cite{billingsley2008probability} to obtain that as $n\rightarrow\infty$ with a high probability,
\begin{align*}
     \bbE\big[ \big( \bmx^\top(\hbeta_m - \beta^*) \big)^2\big] \rightarrow
 \frac{1}{n} \bmx^\top \bM_{X}^{-1}(\beta^*; \cD) \bmx,
\end{align*}
which is combined with \eqref{eq:std_Q1} to get as $n\rightarrow\infty$,
\begin{align}\label{eq:std_Q1_2}
nQ_1 \rightarrow \frac{M}{(M-1)} \bmx^\top \bM_{X}^{-1}(\beta^*; \cD) \bmx,
\end{align}
in probability.

For the term $Q_2$, we obtain from \eqref{eq:normality} that as $n\rightarrow\infty$,
\begin{align*}
\sqrt{n}\bmx^\top(\bar\beta - \beta^*) \rightarrow N\big(0, \frac{1}{M}\bmx^\top\bM_{X}^{-1}(\beta^*, \cD)\bmx\big)
\end{align*}
in distribution. Thus, we can also invoke Theorem 25.12 in \cite{billingsley2008probability} to have as $n\rightarrow\infty$ with a high probability,
\begin{equation}\label{eq:std_Q2_moment}
\begin{aligned}
&n\bbE\big[ \big( \bmx^\top(\bar\beta - \beta^*) \big)^2\big] \rightarrow
\frac{1}{M} \bmx^\top \bM_{X}^{-1}(\beta^*; \cD) \bmx,\\
&n^2\bbE\big[ \big( \bmx^\top(\bar\beta - \beta^*) \big)^4\big] \rightarrow
\frac{3}{M^2} \big(\bmx^\top \bM_{X}^{-1}(\beta^*; \cD) \bmx\big)^2
\end{aligned}
\end{equation}
Additionally, we use Chebyshev's inequality to get for any $a>0$, as $n\rightarrow\infty$,
\begin{align*}
&\bbP\Big(\big|\big(\bmx^\top(\bar \beta - \beta^*)\big)^2 - \frac{1}{nM} \bmx^\top \bM_{X}^{-1}(\beta^*; \cD) \bmx\big| \ge a^2\Big) \\
\le& a^{-2}\bbE\big[\big(\bmx^\top(\bar \beta - \beta^*)\big)^2 - \frac{1}{nM} \bmx^\top \bM_{X}^{-1}(\beta^*; \cD) \bmx\big]^2\\
=& a^{-2}\Big\{\bbE\big[ \big( \bmx^\top(\bar\beta - \beta^*) \big)^4\big] + \big[\frac{1}{nM} \bmx^\top \bM_{X}^{-1}(\beta^*; \cD) \bmx\big]^2 - 2\bbE\big[ \big( \bmx^\top(\bar\beta - \beta^*) \big)^2\big]\cdot\frac{1}{nM} \bmx^\top \bM_{X}^{-1}(\beta^*; \cD) \bmx\Big\}\\
\rightarrow& \frac{2}{a^2n^2M^2} \big(\bmx^\top \bM_{X}^{-1}(\beta^*; \cD) \bmx\big)^2,
\end{align*}
where the last limitation is obtained due to \eqref{eq:std_Q2_moment}. Hence, as $M\rightarrow\infty$, we get
\begin{align}\label{eq:std_Q2_2}
    \big(\bmx^\top(\bar \beta - \beta^*)\big)^2 \rightarrow \frac{1}{nM} \bmx^\top \bM_{X}^{-1}(\beta^*; \cD) \bmx
\end{align}
in probability.

Therefore, by taking \eqref{eq:std_Q1_2} and \eqref{eq:std_Q2_2} back into \eqref{eq:std_decompose}, we have as $M,n\rightarrow\infty$, 
\begin{align*}
    n\std^2 &=n(Q_1 - Q_2)\\
    &\rightarrow \frac{M}{M-1} \bmx^\top \bM_{X}^{-1}(\beta^*; \cD) \bmx - \frac{M}{M-1}\cdot\frac{1}{M} \bmx^\top \bM_{X}^{-1}(\beta^*; \cD) \bmx\\
    &= \bmx^\top \bM_{X}^{-1}(\beta^*; \cD) \bmx,
\end{align*}
in probability.
% Since
% \begin{align*}
%      & \bbE\big[ \big( \bmx^\top(\hbeta_m - \beta^*) \big)^2\big] = 
%  \frac{1}{n} \bmx^\top M_{X}^{-1}(\beta^*; \cD) \bmx\\
%     &  \bbE\big[\bmx^\top(\hbeta_m - \beta^*) (\hbeta_j - \beta^*)^\top \bmx\big] = 0,  \forall j \neq k,
% \end{align*}
% where the equality is obtained by the independence of $\hbeta_m$ and $\hbeta_j$ for any $j,k\in[K]$. By {\color{blue}Assumption XXX and [XXX]}, as $K \rightarrow \infty$, we have
% \begin{align*}
%     \frac{1}{M} \sum_{m=1}^M \Big( \bmx^\top(\hbeta_m - \beta^*) \Big)^2 \rightarrow &  \bbE\big[ \big( \bmx^\top(\hbeta_m - \beta^*) \big)^2\big], \\
%     \frac{1}{K(K-1)} \sum_{k\ne j} \bmx^\top(\hbeta_m - \beta^*) (\hbeta_j - \beta^*)^\top \bmx \rightarrow &\bbE\big[\bmx^\top(\hbeta_m - \beta^*) (\hbeta_j - \beta^*)^\top \bmx\big]. 
% \end{align*}
Then, by invoking Lemma \ref{lemma:closeness_between_Mxbeta}, we finish the proof.
\end{proof}


Therefore, assuming that $\bM_X(\hat\beta_\MLE; \cS)$ is a positive definite matrix in probability for any $k\in[K]$ and $\|\bmx\|_2$ is upper bounded,  we can use $n\std^2$ to approximate the square of uncertainty $\|\bmx\|_{\bM_X(\hat\beta_\MLE; \cS)^{-1}}^2$.




\newpage
\section{Materials}


\begin{proof}
To begin with, the sample covariance matrix $\Sigma_M(\bmx)$ is computed as
\begin{align*} 
(M-1)\Sigma_M(\bmx) &= \sum_{m=1}^M (\hat\bbeta_m - \Tilde\bbeta)^\top \bmx\bmx^\top (\hat\bbeta_m - \Tilde\bbeta)\notag\\
&= \sum_{m=1}^M \big((\hat\bbeta_m - \bbeta^*) - (\Tilde\bbeta - \bbeta^*)\big)^\top \bmx\bmx^\top \big((\hat\bbeta_m - \bbeta^*) - (\Tilde\bbeta - \bbeta^*)\big)\notag\\
&= \sum_{m=1}^M (\hat\bbeta_m - \bbeta^*)^\top \bmx\bmx^\top (\hat\bbeta_m - \bbeta^*) - \frac{1}{M} \sum_{m=1}^M\sum_{l=1}^M (\hat\bbeta_m - \bbeta^*)^\top \bmx\bmx^\top (\hat\bbeta_l - \bbeta^*)\notag\\
&= \frac{M-1}{M}\sum_{m=1}^M (\hat\bbeta_m - \bbeta^*)^\top \bmx\bmx^\top (\hat\bbeta_m - \bbeta^*) - \frac{1}{M} \sum_{m\ne l} (\hat\bbeta_m - \bbeta^*)^\top \bmx\bmx^\top (\hat\bbeta_l - \bbeta^*).
\end{align*}
As $M \xrightarrow[]{} \infty$, 
\begin{align}
    \frac{1}{M}\sum_{m=1}^M (\hat\bbeta_m - \bbeta^*)^\top \bmx\bmx^\top (\hat\bbeta_m - \bbeta^*) \xrightarrow[]{} \bbE[(\hat\bbeta_m - \bbeta^*)^\top \bmx\bmx^\top (\hat\bbeta_m - \bbeta^*)] \\
    \frac{1}{M(M-1)} \sum_{m\ne l} (\hat\bbeta_m - \bbeta^*)^\top \bmx\bmx^\top (\hat\bbeta_l - \bbeta^*) \xrightarrow[]{} \bbE[(\hat\bbeta_m - \bbeta^*)^\top \bmx\bmx^\top (\hat\bbeta_l - \bbeta^*)]
\end{align}
Since $\hat\bbeta_m - \bbeta^*$ and $\hat\bbeta_l - \bbeta^*$ are independent, we have $\bbE[(\hat\bbeta_m - \bbeta^*)^\top \bmx\bmx^\top (\hat\bbeta_l - \bbeta^*)] = 0$, so as $M \xrightarrow[]{} \infty$, 
\begin{align}\label{eq:Sigma_m}
\Sigma_M(\bmx)  \xrightarrow[]{} \bbE\big[ (\hat\bbeta_m - \bbeta^*)^\top \bmx\bmx^\top (\hat\bbeta_m - \bbeta^*)\big].
\end{align}

Therefore, as $M \xrightarrow[]{} \infty$,
\begin{align*}
& s(\hbeta_\MLE; \bmx, y)^\top \Sigma_M(\bmx) s(\hbeta_\MLE; \bmx, y) \\  
\xrightarrow[]{}& s(\hbeta_{\MLE}; ; \bmx, y)^\top \bbE\big[\Sigma_M(\bmx) \big] s(\hbeta_{\MLE}; \bmx, y)\\
=& s(\hbeta_{\MLE}; \bmx, y)^\top \bbE_{\hat\bbeta_m}\big[ (\hat\bbeta_m - \bbeta^*)^\top \bmx\bmx^\top (\hat\bbeta_m - \bbeta^*) \big] s(\hbeta_{\MLE}; \bmx, y)\\
=& \TRACE\Big\{\psi(\hbeta_{\MLE}; \bmx, y)\otimes (\bmx\bmx^\top) \cdot \bbE_{\hat\bbeta_m}\big[ (\hat\bbeta_m - \bbeta^*)(\hat\bbeta_m - \bbeta^*)^\top \big]\Big\},
\end{align*}
By using the asymptotic normality of $\hat \bbeta_m$ [{\color{blue}Reference}]:
$$
\sqrt{n}(\hat \bbeta_m-\bbeta^*) \rightarrow \cN(0, M_X^{-1}(\bbeta^*;\cD)),
$$
we obtain that as $M \xrightarrow[]{} \infty$ and $n \xrightarrow[]{} \infty$,
\begin{align}
n \TRACE(\psi(\hbeta;\bmx, y)\Sigma_M(\bmx))  &\xrightarrow[]{} \TRACE\Big\{\psi(\hbeta_{\MLE};\bmx)\otimes (\bmx\bmx^\top) M_X(\beta^*;\cD)^{-1} \Big\},
\end{align}
{\color{blue}(the two are the same?)We finish the proof by noting $M_X(\hbeta_\MLE;\cS)$ converging to the positive definite matrix $M_X(\beta^*;\cD)^{-1}$}.
    
\end{proof}

\section{Additional Results}



\begin{table}[t]
\centering
\footnotesize	
   \begin{tabular}{c|c|c|c|c|c}
\hline 
\multirow{2}{*}{Sampling Method } & \multirow{2}{*}{Reweighting} & \multicolumn{2}{c|}{Two Class} & \multicolumn{2}{c}{Ten Class}\tabularnewline
\cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 &  & 300 & 1000 & 300 & 1000\tabularnewline
\hline 
Random & Equal& 88.31 (1.39) & 94.15 (0.72) & 58.35 (0.39) & 71.79 (0.54)\tabularnewline
\hline 
Uncertainty with y & Equal &60.81 (4.95)  &  93.61 (0.66)& 47.31 (0.82) &68.03 (0.84)  \tabularnewline
\hline 
Uncertainty with y & Inverse Uncertainty& 79.52 (5.60)& 94.27 (1.07)&48.92 (1.41)&
67.08 (1.53)\tabularnewline
\hline 
Uncertainty with y (Clip) & Equal & 86.61 (1.16)	 & 94.57 (0.81) & 57.3 (0.69) & 72.0 (0.5)\tabularnewline
\hline 
% Uncertainty with y(Clip) & Inverse Uncertainty &83.57 (1.38) &86.42 (1.18) &53.85 (1.07) & 67.9 (1.02)\\
% \hline
Uncertainty with y (Clip) & Inverse Uncertainty (Clip) & 90.02 (0.61) & 95.07 (0.41) & 60.8 (0.99) & 73.22 (0.46)
\tabularnewline
\hline 
Random without y &  Equal  & 88.08 (1.54)	&94.17 (0.42) &57.85 (0.25)	&71.89 (0.41)\\
\hline
Uncertainty without y & Equal  &87.18 (0.94)	&95.45 (0.69) &52.67 (1.51)	&72.11 (0.95)\\
\hline
Uncertainty without y & Inverse Uncertainty &88.38 (0.7)&	95.04 (0.45) & 53.61 (1.26)	&72.4 (0.37)\\
% Uncertainty without y & Equal &86.34 (2.07)	  & 95.42 (0.61) & 54.04 (0.51) & 71.45 (0.49)\tabularnewline
\hline 
Uncertainty  without y (Clip) & Equal & 89.6 (0.56) &  95.39 (0.31)& 58.26 (0.64)	&72.18 (0.86) \tabularnewline
\hline 
% Uncertainty without y (Clip)& Inverse Uncertainty & 87.63 (1.24)
% & 95.14 (0.42) & 57.65 (0.67)& 71.53 (0.72)\\
% \hline
Uncertainty without y (Clip) & Inverse Uncertainty (Clip)  & 89.7 (0.27) & 95.56 (0.23) & 60.7 (0.72)&	72.95 (0.69)\tabularnewline
\hline 
\end{tabular}
    \caption{\label{tab:vanilla_inferior}This table illustrates the performance of different sampling methods on binary classification and ten-class classification tasks for ResNet20w on Cifar. 300/1000 means 300/1000 samples for each class. We run each method 5 times and report the mean and std for them.}
\end{table}
\begin{table}[H]
    \centering
    \scriptsize
    \begin{tabular}{c|c|c|c|c|c|c}
\hline 
\multirow{2}{*}{Model} & \multirow{2}{*}{Sampling Method} & \multirow{2}{*}{Reweighting} & \multicolumn{2}{c|}{Two Class} & \multicolumn{2}{c}{Ten Class}\tabularnewline
\cline{4-7} \cline{5-7} \cline{6-7} \cline{7-7} 
 &  &  & 300 & 1000 & 300 & 1000\tabularnewline
\hline 
\multirow{7}{*}{ResNet56} & Random & Equal & 88.2 (0.8) & 92.96 (0.75) & 56.45 (1.41) &72.19 (0.6) \tabularnewline
\cline{2-7} \cline{3-7} \cline{4-7} \cline{5-7} \cline{6-7} \cline{7-7} 
 & Uncertainty with y(Clip) & Equal & 86.37 (1.5) &  94.34 (0.46)& 55.86 (0.29) &72.56 (0.73) \tabularnewline
\cline{2-7} \cline{3-7} \cline{4-7} \cline{5-7} \cline{6-7} \cline{7-7} 
 & Uncertainty with y(Clip) & Inverse Uncertainty (Clip) & 88.75 (1.51) &  94.87 (1.01)& 59.44 (0.51) & 74.89 (0.55)\tabularnewline
\cline{2-7} \cline{3-7} \cline{4-7} \cline{5-7} \cline{6-7} \cline{7-7} 
 & Uncertainty without y(Clip) & Equal & 88.75 (0.86) & 94.52 (0.93) &57.41 (0.92) &72.73 (0.36) \tabularnewline
\cline{2-7} \cline{3-7} \cline{4-7} \cline{5-7} \cline{6-7} \cline{7-7} 
 & Uncertainty without y(Clip) & Inverse Uncertainty (Clip) &  89.71 (1.24)& 94.41 (1.12) &  59.17 (0.79) & 73.51 (0.74)\tabularnewline
\hline 
\multirow{7}{*}{MobileV2} & Random & Equal &  88.63 (1.06)&  95.03 (0.57)& 57.87 (1.26) & 73.66 (0.42)\tabularnewline

\cline{2-7} \cline{3-7} \cline{4-7} \cline{5-7} \cline{6-7} \cline{7-7} 
 & Uncertainty with y(Clip) & Equal & 86.62 (1.67) & 94.46 (0.24) & 57.62 (1.09) & 74.7 (0.61)\tabularnewline
\cline{2-7} \cline{3-7} \cline{4-7} \cline{5-7} \cline{6-7} \cline{7-7} 
 & Uncertainty with y(Clip) & Inverse Uncertainty (Clip) & 88.75 (0.84) & 95.76 (0.41) & 59.63 (0.7) & 75.37 (0.33)\tabularnewline
\cline{2-7} \cline{3-7} \cline{4-7} \cline{5-7} \cline{6-7} \cline{7-7} 
 & Uncertainty without y(Clip) & Equal & 87.86 (1.11) & 94.59 (0.34) & 58.2 (0.65) & 74.31 (0.68)\tabularnewline
\cline{2-7} \cline{3-7} \cline{4-7} \cline{5-7} \cline{6-7} \cline{7-7} 
 & Uncertainty without y(Clip) & Inverse Uncertainty (Clip) & 89.24 (0.43 & 95.51 (0.37) & 59.77 (0.62)  &74.75 (0.42) \tabularnewline
\hline 
\multirow{7}{*}{DenseNet121} & Random & Equal & 87.87 (0.99) &  94.3 (0.54)& 65.04 (0.36)& 78.85 (0.4)\tabularnewline
\cline{2-7} \cline{3-7} \cline{4-7} \cline{5-7} \cline{6-7} \cline{7-7} 
 & Uncertainty with y(Clip) & Equal & 85.05 (0.94) &  94.69 (0.67)&  64.36 (0.68)& 79.72 (0.29)\tabularnewline
\cline{2-7} \cline{3-7} \cline{4-7} \cline{5-7} \cline{6-7} \cline{7-7} 
 & Uncertainty with y(Clip) & Inverse Uncertainty (Clip) & 88.8 (1.49) &  95.69 (0.25)&66.38 (0.32)  &80.17 (0.26) \tabularnewline
\cline{2-7} \cline{3-7} \cline{4-7} \cline{5-7} \cline{6-7} \cline{7-7} 
 & Uncertainty without y(Clip) & Equal & 88.03 (0.7) & 95.86 (0.35) &  64.55 (0.68) &79.47 (0.33) \tabularnewline
\cline{2-7} \cline{3-7} \cline{4-7} \cline{5-7} \cline{6-7} \cline{7-7} 
 & Uncertainty without y(Clip) & Inverse Uncertainty (Clip) & 88.17 (1.07) & 96.11 (0.76) &  66.46 (0.25)& 80.13 (0.22)\tabularnewline
\hline 

\end{tabular}
 \caption{\label{tab:cifar_net} This table illustrates the performance of different sampling methods on binary classification and ten-class classification tasks for ResNet56, MobileNetV2 and DenseNet121 on Cifar. 300/1000 means 300/1000 samples for each class. We run each method 5 times and report the mean and std for them. (fig: x axis: models, two subfigures: 300/1000)}
\end{table}



\begin{table}[htb]
    \centering
    \begin{tabular}{c|c|c|c|c}
\hline 
\multirow{2}{*}{Sampling Method} & \multirow{2}{*}{Reweighting} & \multicolumn{3}{c}{Two Class}\tabularnewline
\cline{3-5} \cline{4-5} \cline{5-5} 
 &  & 1000 & 2000 & 5000\tabularnewline
\hline 
Random & Equal & 77.81 (0.66) & 82.12 (0.68)  & 85.2 (0.46)\tabularnewline
\hline  
Uncertainty with y(Clip) & Equal & 74.05 (1.21)	& 80.98 (0.74)	&85.3 (0.27)  \tabularnewline
\hline 
Uncertainty with y(Clip) & Inverse Uncertainty (Clip) &  79.58 (0.66)&	84.13 (0.47)	&86.93 (0.21) \tabularnewline
\hline 
Uncertainty without y(Clip) & Equal & 79.05 (0.55)	& 82.19 (0.72) &  85.5 (0.21)\tabularnewline
\hline 
Uncertainty without y(Clip) & Inverse Uncertainty (Clip) & 80.04 (0.93)	&82.81 (0.57)   & 85.85 (0.2)\tabularnewline
\hline 
\end{tabular}
 \caption{\label{tab:imdb} This table illustrates the performance of different sampling methods on binary classification  tasks for GRU-based model on IMDB. 1000/2000/5000 means 1000/2000/5000 samples for each class. We run each method 5 times and report the mean and std for them.}
\end{table}


\begin{table}[htb]
    \centering
    \footnotesize
   \begin{tabular}{c|c|c|c|c|c}
\hline 
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Sampling Method} & \multirow{2}{*}{Reweighting} & \multicolumn{3}{c}{Ten Class}\tabularnewline
\cline{4-6} \cline{5-6} \cline{6-6} 
 &  &  & 300  & 1000  & 2000\tabularnewline
\hline 
\multirow{7}{*}{SVHN} & Random  & Equal  & 89.96 (0.69) &  94.13 (0.15)	&95.54 (0.12) \tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & Uncertainty with y(Clip)  & Equal  & 90.26 (0.43) & 95.22 (0.2)	 & 96.34 (0.09)\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & Uncertainty with y(Clip)  & Inverse Uncertainty (Clip)  & 91.55 (0.38) & 95.9 (0.2)	 & 96.67 (0.05)\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & Uncertainty without y(Clip)  & Equal  & 90.66 (0.42) & 95.32 (0.19)	&96.47 (0.21)  \tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & Uncertainty without y(Clip)  & Inverse Uncertainty (Clip)  &  90.92 (0.39)& 95.48 (0.22) & 96.61 (0.07)\tabularnewline
\hline 
\multirow{7}{*}{Place365} & Random  & Equal  & 70.83 (2.58) &84.97 (1.95)	&90.0 (0.71)  \tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & Uncertainty with y(Clip)  & Equal  & 71.6 (2.22) &85.73 (1.46)  & 90.67 (0.45)\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & Uncertainty with y(Clip)  & Inverse Uncertainty (Clip)  &72.43 (3.0) &  86.87 (0.74) & 91.87 (0.63)\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & Uncertainty without y(Clip)  & Equal  & 72.47 (2.59) & 87.27 (0.09)	 & 90.97 (0.17)\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & Uncertainty without y(Clip)  & Inverse Uncertainty (Clip)  & 71.87 (1.64) &86.37 (1.11)	  & 91.47 (0.33)\tabularnewline
\hline 
\end{tabular}
 \caption{\label{tab:multi_more} This table illustrates the performance of different sampling methods on ten-class classification tasks for ResNet20 on SVHN and  ResNet18 model on Place365. 300/1000/2000 means 300/1000/2000 samples for each class. We run each method 5 times and report the mean and std for SVHN and 3 times for Place365 . (fig: x axis: 300/1000/2000, two subfigures:SVHN/Places))}
\end{table}

\begin{table}[htb]
    \centering
    \footnotesize
   \begin{tabular}{c|c|c|c|c|c}
\hline 
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Sampling Method} & \multirow{2}{*}{Reweighting} & \multicolumn{3}{c}{Ten Class}\tabularnewline
\cline{4-6} \cline{5-6} \cline{6-6} 
 &  &  & 300  & 1000  & 2000\tabularnewline
\hline 
\multirow{7}{*}{CIFAR-Worst} & Random  & Equal  & 40.89 (1.11) & 54.03 (0.46)	& 58.58 (0.3) \tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & Uncertainty with y(Clip)  & Equal  & 40.91 (0.97) & 53.86 (0.9)	& 59.08 (1.0) \tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & Uncertainty with y(Clip)  & Inverse Uncertainty (Clip)  & 46.08 (0.75) & 59.47 (0.81)	 & 63.13 (0.8)\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & Uncertainty without y(Clip)  & Equal  & 40.54 (1.24) & 54.2 (0.55)	&59.2 (0.63)  \tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & Uncertainty without y(Clip)  & Inverse Uncertainty (Clip)  &  41.53 (0.76)	& 54.51 (0.78) & 58.6 (0.52)\tabularnewline
\hline 
\multirow{7}{*}{CIFAR-Agg} & Random  & Equal  & 54.99 (1.11) &  68.88 (0.56)	& 74.76 (0.47)\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & Uncertainty with y(Clip)  & Equal  & 55.31 (1.26) & 68.76 (0.35)	 & 74.66 (0.13)\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & Uncertainty with y(Clip)  & Inverse Uncertainty (Clip)  & 59.71 (0.38) & 71.99 (0.19) & 77.44 (0.15)\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & Uncertainty without y(Clip)  & Equal  & 55.35 (0.49) & 69.07 (0.47)	&75.17 (0.41)  \tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & Uncertainty without y(Clip)  & Inverse Uncertainty (Clip)  & 57.11 (0.3)	&  69.83 (0.37) & 75.48 (0.48)\tabularnewline
\hline 
\end{tabular}
 \caption{\label{tab:cifar_n} This table illustrates the performance of different sampling methods on ten-class classification tasks for ResNet20 on SVHN and  ResNet18 model on Place365. 300/1000/2000 means 300/1000/2000 samples for each class. We run each method 5 times and report the mean and std for them. (fig: x axis: 300/1000/2000, two subfigures:agg/worst)) }
\end{table}


\begin{table}[htb]
    \centering
    \begin{tabular}{c|c|c|c|c}
\hline 
\multirow{2}{*}{Sampling Method} & \multirow{2}{*}{Reweighting} & \multicolumn{2}{c}{Ten Class}\tabularnewline
\cline{3-5} \cline{4-5}  \cline{5-5}  
 &  &  300&1000 & 2000\tabularnewline
\hline 
Random with $Y$ & Equal & 58.35 (0.39)&71.79 (0.54)  &78.24 (0.41)\tabularnewline
\hline  
Uncertainty with $Y$(Clip) & Equal& 58.28 (0.73)&72.19 (0.36)  &	78.96 (0.24) \tabularnewline
\hline 
Uncertainty with y(Clip) & Inverse Uncertainty (Clip) &60.88 (0.39) & 73.24 (0.6) &	79.49 (0.06) \tabularnewline
\hline 
Uncertainty without y(Clip) & Equal & 58.13 (1.02)& 72.69 (0.57) &78.94 (0.21)	\tabularnewline
\hline 
Uncertainty without y(Clip) & Inverse Uncertainty (Clip) &58.88 (0.53) &72.21 (0.31)  & 78.96 (0.28) \tabularnewline
\hline 
\end{tabular}
 \caption{\label{tab:cifar10_dropout} This table illustrates the performance of different sampling methods on ten-class classification  tasks for ResNet20 on CIFAR. 1000/2000/5000 means 1000/2000/5000 samples for each class. We run each method 5 times and report the mean and std for them. Here we use dropout to estimate the uncertainty. (Figure dropout VS 10 models, bootstrap)}
\end{table}




\begin{figure}[H]
\centering
\begin{minipage}[t]{0.48\textwidth}
\centering
\includegraphics[width=6cm]{fig/compawy.pdf}
\caption*{(a)Comparison on CIFAR10 with Y.}
\end{minipage}
\begin{minipage}[t]{0.48\textwidth}
\centering
\includegraphics[width=6cm]{fig/compawoy.pdf}
\caption*{(b)Comparison on CIFAR10 without Y.}
\end{minipage}
% \caption{}
\caption{Results for Cifar10 with comparison.\label{cifar10_compare}For Badge with 3000 samples, the performance is lower than 50, so the bar is clipped in our figures.}

\end{figure}


\begin{figure}[H]
\centering
\begin{minipage}[t]{0.48\textwidth}
\centering
\includegraphics[width=6cm]{fig/cifaracompawy.pdf}
\caption*{(a)Comparison on CIFAR10 Aggre with Y.}
\end{minipage}
\begin{minipage}[t]{0.48\textwidth}
\centering
\includegraphics[width=6cm]{fig/cifaracompawoy.pdf}
\caption*{(b)Comparison on CIFAR10 Aggre without Y.}
\end{minipage}
\caption{Results for Cifar10 Aggregation with comparison.\label{cifar10a_compare}}
\end{figure}


\begin{figure}[H]
\centering
\begin{minipage}[t]{0.48\textwidth}
\centering
\includegraphics[width=6cm]{fig/cifarwcompawy.pdf}
\caption*{(a)Comparison on CIFAR10 Worst with Y.}
\end{minipage}
\begin{minipage}[t]{0.48\textwidth}
\centering
\includegraphics[width=6cm]{fig/cifarwcompawoy.pdf}
\caption*{(b)Comparison on CIFAR10 Worst without Y.}
\end{minipage}
\caption{Results for Cifar10 Worse with comparison.\label{cifar10w_compare}}
\end{figure}


\begin{figure}[H]
\centering
\begin{minipage}[t]{0.48\textwidth}
\centering
\includegraphics[width=6cm]{fig/cifar100compawy.pdf}
\caption*{(a)Comparison on CIFAR100  with Y.}
\end{minipage}
\begin{minipage}[t]{0.48\textwidth}
\centering
\includegraphics[width=6cm]{fig/cifar100compawoy.pdf}
\caption*{(b)Comparison on CIFAR100  without Y.}
\end{minipage}
\caption{\label{cifar100}Results of THOSE on CIFAR100 with compared methods.}
\end{figure}


\newpage
\section{Additional simulation}
we consider that the total mis-specification level is upper bounded as $\sum_{\bx}|\zeta(\bx)|~\leq~C$.
Denoting $C_1 = \zeta(\bmx_1)$, $C_2 = \zeta(\bmx_2)$, and $C_3 = \zeta(\bmx_3)$, we consider three cases with mis-specification in addition to an well specified case:
\begin{itemize}
    \item[(1)] There is mis-specification  on $\bmx_1$, i.e., $n_1C_1=3000$, $C_2=0$, and $C_3=0$,
    \item[(2)] There is mis-specification   on $\bmx_2$, i.e., $C_1=0$, $n_2C_2=3000$, and $C_3=0$,
    \item[(3)] There is mis-specification   on $\bmx_3$, i.e.,  $C_1=0$, $C_2=0$, and $n_3C_3=3000$.
    \item[(4)] There is no mis-specification ,  i.e.,  $C_1=0$, $C_2=0$, and $C_3=0$. 
\end{itemize}
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.6]{fig/Simulation_of_clip_.pdf}
    \caption{Simulation of uncertainty Clip}
    \label{fig:mis-specification_simulation}
\end{figure}
We sub-sample 3,000 samples out of totally 201,000 samples and obtain $\bar \beta$ according to Algorithm~\ref{algo:linear_those_active}. We evaluate the error of the prediction $\sum_{\bx} |\bx^\top(\bar \beta - \beta^*)|$ on the test set which also contains 1,000 numbers of $\bmx_1$, 100,000 numbers of $\bmx_2$ and $\bmx_3$, respectively. The simulation results in Figure~\ref{fig:mis-specification_simulation} show that when there is mis-specification on $\bmx_2$, $\bmx_3$ or there is no mis-specification, uncertainty sampling leads to better performance than random sampling.  When there is mis-specification on $\bmx_1$, directly applying Algorithm~\ref{algo:linear_those_active} leads to much higher prediction error than random sampling.

\section{Some Tables}

\begin{table}[H]
\centering
\footnotesize	
   \begin{tabular}{c|c|c|c|c|c}
\hline 
\multirow{2}{*}{Sampling Method } & \multirow{2}{*}{Reweighting} & \multicolumn{2}{c|}{Two Class} & \multicolumn{2}{c}{Ten Class}\tabularnewline
\cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 &  & 300 & 1000 & 300 & 1000\tabularnewline
\hline 
Random with y & Equal & 88.31 (1.39) & 94.15 (0.72) & 58.35 (0.39) & 71.79 (0.54)\tabularnewline
\hline 
Uncertainty with y & Equal &60.81 (4.95)  &  93.61 (0.66)& 47.31 (0.82) &68.03 (0.84) \tabularnewline
\hline
Uncertainty with y & Inverse Uncertainty& 79.52 (5.60)& 94.27 (1.07)&48.92 (1.41)&
67.08 (1.53)\tabularnewline
\hline 
Random without y &  Equal  & 88.08 (1.54)	&94.17 (0.42) &57.85 (0.25)	&71.89 (0.41)\\
\hline
Uncertainty without y & Equal  &87.18 (0.94)	&95.45 (0.69) &52.67 (1.51)	&72.11 (0.95)\\
\hline
Uncertainty without y & Inverse Uncertainty &88.38 (0.7)&	95.04 (0.45) & 53.61 (1.26)	&72.4 (0.37)\\
\hline
\end{tabular}
    \caption{This table illustrates the performance of different sampling methods on binary classification and ten-class classification tasks for ResNet20 on CIFAR. 300/1000 means 300/1000 samples for each class. We run each method 5 times and report the mean and std for them.}
\label{tab:vanilla_inferior_results}
\end{table}


\begin{table}[H]
\centering
\begin{tabular}{c|c|c|c}
\hline 
Sampling Method & Reweight & 600 & 2000\tabularnewline
\hline 
Random with Y & Equal & 88.31 (1.39)  & 94.15 (0.72)\tabularnewline
\cline{2-4} \cline{3-4} \cline{4-4} 
Uncertainty with Y & Equal & 86.61 (1.16)  & 94.57 (0.81)\tabularnewline
\cline{2-4} \cline{3-4} \cline{4-4} 
Uncertainty with Y & Inverse Uncertainty & 90.02 (0.61)  & 95.07 (0.41)\tabularnewline
\cline{2-4} \cline{3-4} \cline{4-4} 
Dropout with Y & Equal &  88.55 (0.85)& 95.11 (0.66)\tabularnewline
\cline{2-4} \cline{3-4} \cline{4-4} 
Dropout with Y & Inverse Uncertainty &  89.66 (1.09)& 95.74 (0.63)\tabularnewline
\cline{2-4} \cline{3-4} \cline{4-4} 
Bootstrap with Y & Equal & 89.02 (0.81)	 & 94.77 (0.7) \tabularnewline
\cline{2-4} \cline{3-4} \cline{4-4} 
Bootstrap with Y & Inverse Uncertainty & 89.29 (1.57) & 95.08 (0.51)\tabularnewline
\hline 
Random without Y & Equal & 88.08 (1.54)  & 94.17 (0.42)\tabularnewline
\cline{2-4} \cline{3-4} \cline{4-4} 
Uncertainty without Y & Equal &89.6 (0.56) & 95.39 (0.31)\tabularnewline
\cline{2-4} \cline{3-4} \cline{4-4} 
Uncertainty without Y & Inverse Uncertainty &  89.7 (0.27) & 95.56(0.23) \tabularnewline
\cline{2-4} \cline{3-4} \cline{4-4} 
Dropout without Y & Equal & 89.0 (0.8) &94.75 (0.94) \tabularnewline
\cline{2-4} \cline{3-4} \cline{4-4} 
Dropout without Y & Inverse Uncertainty & 88.9 (0.76) & 94.71 (0.56)\tabularnewline
\cline{2-4} \cline{3-4} \cline{4-4} 
Bootstrap without Y & Equal & 88.66 (0.46) & 94.66(0.75)\tabularnewline
\cline{2-4} \cline{3-4} \cline{4-4} 
Bootstrap without Y & Inverse Uncertainty & 88.99 (0.76) &94.66(0.75)  \tabularnewline
\hline 
\end{tabular}
\caption{Comparison of different type of uncertainty on CIFAR binary setting. 600/2000 means sample 600/2000 instances from 8000 instances in all.}
\end{table}

\paragraph{Vanilla uncertainty sampling may suffer from model misspecification.}

By view  Table.~\ref{tab:vanilla_inferior}, we have several observations.
Firstly, clipping the uncertainty during training can boost the performance for all the settings by a significant margin.
In addition, using clipping during reweighting is also very effective.
Using clipping  for sampling and reweighting can make the trained models better than all the comparing variants significantly.
To get more understanding of the clipping, we visualize the distribution of the uncertainty for the with-y type on CIFAR binary setting and ResNet20.
The  histogram is shown in Figure.~\ref{fig:uncertainty_histogram}, we can find that most of the samples have a relatively small uncertainty value between 0 and 0.1. 
However, some samples have values greater than 4.
The difference in scale leads to a problem. 
The highly uncertain instances are much more likely to be selected, which let the sampled set difficult to learn when the whole sample size is small.
We illustrate the uncertainty of 2000 instances sampled from the distribution.
Figure.~\ref{fig:uncertainty_histogram_sampled} shows the sampled histogram.
We can find that the sampled instances have a higher ratio of samples with uncertainty greater than 1.
Figure.~\ref{fig:uncertainty_histogram_0_01} shows the value between 0 and 0.1.
By observation, we can find that some of the uncertainty values are even smaller than 0.01, which leads to an inverse uncertainty reweight greater than 100, it also explains why we also need to clip the reweight intuitively.

